Who Checks the Checkers? Exploring Source Credibility in Twitter's Community Notes

In recent years, the proliferation of misinformation on social media platforms has become a significant concern. Initially designed for sharing information and fostering social connections, platforms like Twitter (now rebranded as X) have also unfortunately become conduits for spreading misinformation. To mitigate this, these platforms have implemented various mechanisms, including the recent suggestion to use crowd-sourced non-expert fact-checkers to enhance the scalability and efficiency of content vetting. An example of this is the introduction of Community Notes on Twitter. While previous research has extensively explored various aspects of Twitter tweets, such as information diffusion, sentiment analytics and opinion summarization, there has been a limited focus on the specific feature of Twitter Community Notes, despite its potential role in crowd-sourced fact-checking. Prior research on Twitter Community Notes has involved empirical analysis of the feature's dataset and comparative studies that also include other methods like expert fact-checking. Distinguishing itself from prior works, our study covers a multi-faceted analysis of sources and audience perception within Community Notes. We find that the majority of cited sources are news outlets that are left-leaning and are of high factuality, pointing to a potential bias in the platform's community fact-checking. Left biased and low factuality sources validate tweets more, while Center sources are used more often to refute tweet content. Additionally, source factuality significantly influences public agreement and helpfulness of the notes, highlighting the effectiveness of the Community Notes Ranking algorithm. These findings showcase the impact and biases inherent in community-based fact-checking initiatives.

==> Sections/checklist.tex <==
\section{Ethics checklist}

\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    \answerYes{Yes, this work follows the required principles.}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes all contributions listed in the abstract and introduction accurately reflect the paper's contribution. See Section \ref{sec:intro}.}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerYes{Yes, we explain the aims and how our proposed methodological tools helps us reach those aims. See Section \ref{sec:analysis}.}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerYes{Yes, we clarify that our data is limited to English. See Section \ref{sec:data}.}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, with each data processing step we highlight limitations of our work. See Sections \ref{sec:data} and \ref{sec:analysis}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Yes, we highlight that the unbalanced bias of sources on Community Notes might negatively affect the neutrality of fact-checking on the platform. See Section \ref{sec:analysis}.}
      \item Did you discuss any potential misuse of your work?
    \answerYes{Yes, we highlight that in order to mitigate any misuse, we indicate each step taken in our research. See Section \ref{sec:data}.}
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerYes{Yes, we documented thoroughly all of our data and models. In addition as the data is already anonymized by the platform, no additional data anonymization was needed. See Sections \ref{sec:data} and \ref{sec:analysis}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes, we have read the ethics review guidelines and believe our paper conforms to them.}
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    \answerNA{Not applicable as we were conducting an exploratory work.}
  \item Have you provided justifications for all theoretical results?
    \answerNA{Not applicable as we were conducting an exploratory work.}
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    \answerNA{Not applicable as we were conducting an exploratory work.}
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    \answerNA{Not applicable as we were conducting an exploratory work.}
  \item Did you address potential biases or limitations in your theoretical framework?
    \answerNA{Not applicable as we were conducting an exploratory work.}
  \item Have you related your theoretical results to the existing literature in social science?
    \answerNA{Not applicable as we were conducting an exploratory work.}
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    \answerNA{Not applicable as we were conducting an exploratory work.}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{Not applicable as we did not have any theoretical proofs}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{Not applicable as we did not have any theoretical proofs}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Yes, we introduce all of our code, data and instructions of our model which allows to reproduce the main experimental results. See Sections \ref{sec:data} and \ref{sec:analysis}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes, we thorougly explain all of the training details. See Section \ref{sec:analysis}.}
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes, we included bootstrapped 99\% intervals to our results. See Section \ref{sec:analysis}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{No, as our data and model were sufficiently small that a laptop CPU could handle it, we did not see the need to specify these details.}
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    \answerYes{Yes, we explain the interpretability of our results and explain results against that. See Section \ref{sec:analysis}.}
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
    \answerNo{No, as the classification result was not itself the focus of our model, we did not discuss it. Our focus was the model coefficients, which have no additional ''cost'' in this sense. We additionally calculated 99\% confidence intervals to make our results more robust. See Section \ref{sec:analysis}.}
  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes, the existing asset we used was the original Community Notes data, which we also cited. See Section \ref{sec:data}.}
  \item Did you mention the license of the assets?
    \answerYes{Yes, we mention that the data is publicly released by Twitter under a royalty free licence. See Section \ref{sec:data}.}
  \item Did you include any new assets in the supplemental material or as a URL?
    \answerNo{No, we did not use any new assets.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{No, we did not mention it as we used data from a third party. As Twitter follows strict data processing regulation and also collects data only of registered users, then all required consent collection is already done by the platform.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Yes, we mention that the data we use is anonymized. See Section \ref{sec:data}.}
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR (see \citet{fair})?
\answerNA{Not applicable as we did not release a new dataset.}
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset (see \citet{gebru2021datasheets})? 
\answerNA{Not applicable as we did not release a new dataset.}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerNA{Not applicable as we did not directly conduct research with human subjects}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerNA{Not applicable as we did not directly conduct research with human subjects}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{Not applicable as we did not directly conduct research with human subjects}
   \item Did you discuss how data is stored, shared, and deidentified?
   \answerNA{Not applicable as we did not directly conduct research with human subjects}
\end{enumerate}

\end{enumerate}
